An Embarrassingly Simple Backdoor Attack on Self-supervised Learning

As a new paradigm in machine learning, self-supervised learning (SSL) is capable of learning high-quality representations of complex data without relying on labels. In addition to eliminating the need for labeled data, research has found that SSL improves the adversarial robustness over supervised learning since lacking labels makes it more challenging for adversaries to manipulate model predictions. However, the extent to which this robustness superiority generalizes to other types of attacks remains an open question. We explore this question in the context of backdoor attacks. Specifically, we design and evaluate CTRL, an embarrassingly simple yet highly effective self-supervised backdoor attack. By only polluting a tiny fraction of training data (<= 1%) with indistinguishable poisoning samples, CTRL causes any trigger-embedded input to be misclassified to the adversary's designated class with a high probability (>= 99%) at inference time. Our findings suggest that SSL and supervised learning are comparably vulnerable to backdoor attacks. More importantly, through the lens of CTRL, we study the inherent vulnerability of SSL to backdoor attacks. With both empirical and analytical evidence, we reveal that the representation invariance property of SSL, which benefits adversarial robustness, may also be the very reason making \ssl highly susceptible to backdoor attacks. Our findings also imply that the existing defenses against supervised backdoor attacks are not easily retrofitted to the unique vulnerability of SSL.

==> background.tex <==
\section{Preliminaries}
\label{sec:background}

We first introduce fundamental concepts and assumptions used throughout the paper.
% The important notations are summarized in Table~\ref{tab:symbol}.

% \begin{table}[!ht]{\footnotesize
%     \centering
%       \renewcommand{\arraystretch}{1.1}
%     \begin{tabular}{r|l}
%     {Notation} & {Definition}\\
%     \hline
%     \hline
%     $x, x_*$ & clean input, trigger input \\
%     $x_i$ & $i$-th example\\
%     $v_i, v'_i$ &  different augmented views of $x_i$ \\
%     $z_i$ &  (normalized) representation of $v_i$\\
%     $X$, $Y$ & input space, output space \\
%     $r$ & trigger \\
%     $D,D_*$ & clean training dataset, poisoned training  dataset \\
% %    $m$ & mask ($\alpha$ for each pixel) \\
%     $f, f_*$ & benign model, trojan model\\
%     $g$ & downstream classifier\\
%     %$\psi$ & perturbation function \\
%     $t$ & adversary's target class \\
%     \end{tabular}
%     \caption{Symbols and notations. \label{tab:symbol}}}
% \end{table}
    
\subsection{Self-supervised Learning}

\deleted{Deep neural networks (\dnns) represent a class of machine learning models to learn high-level abstractions for complex data. In a predictive task,} a \dnn $h_\theta$ (parameterized by $\theta$) encodes a function $h_{\theta}: \sR^n \rightarrow \sS^m$, where $n$ and $m$ denote the input dimensionality and the number of classes. A \dnn typically comprises two parts $h = g \circ f$ wherein $f$ is the encoder that extracts representations from given inputs while $g$ is the classifier that maps such representations to output classes. Under the supervised setting, to train a \dnn $h$, the training algorithm uses a training set $\gD$, in which each instance $(x, y)$ comprises input $x$ and its ground-truth label $y$, and optimizes $h$'s parameters $\theta$ with respect to a loss function $\sE_{(x,y) \in \gD} \,\ell(h_\theta(x), y)$ (\meg, the cross entropy of $h_\theta(x)$ and $y$). 

However, supervised learning is inapplicable when data labeling is scarce or expensive\deleted{ (\meg, massive data crawled from the Web)}. Recently, self-supervised learning (\ssl) is emerging as a new paradigm for such settings. Using the supervisory signals from the data itself, \ssl trains a high-quality encoder $f$, which can then be integrated with a downstream classifier $g$ and fine-tuned with weak supervision to form the end-to-end model.

Conceptually, \ssl can be categorized as generative and contrastive \cite{jaiswal2020survey}. In this paper, we mainly focus on contrastive learning. \deleted{ that performs representation learning by optimizing {\em alignment} -- aligning the latent representations of the same sample under varying data augmentations (\mie, ``positive pairs''), 
and/or {\em uniformity} -- separating the representations of the augmented views of different samples (\mie, ``negative pairs'').} Below, we introduce three representative methods of them, as illustrated in Figure\mref{figure:contra}.



% Supervised learning uses a great number of labeled training data to learn a function, which can map an input to a output. Formally, the goal of supervised learning is to learn a function $f_\theta: X \rightarrow Y$, where $X$ denotes the input space, $Y$ denotes the output space, and $\theta$ denotes the parameter.


% Take the classification task as an example. Given a training dataset $D = \{(x_1, y_1), ..., (x_N, y_N) \}$, of which each input-label pair $(x_i, y_i) \in X \times Y$,  $x_i$ is an input example, and $y_i$ is the corresponding label. The supervised learning algorithm aims to find the optimal parameter $\theta^*$ such that:
% $$
% \theta^* = \min_{\theta} \mathbb{E}_{(x_i, y_i) \in  D} [\ell(x_i, y_i; \theta)],
% $$
% where $\ell$ is a loss function (e.g., cross entropy).


% \subsection{Self-supervised Learning}
\begin{figure}[!ht]
	\centerline{\includegraphics[width=0.9\columnwidth]{./figures/contrast.pdf}}
	\caption{Illustration of representative contrastive learning methods.} 
	%\jiang{view1 is same to input. We should modify the notations. }
	\label{figure:contra}
\end{figure}

% \noindent 

\vspace{1pt}
\underline{\em SimCLR}\mcite{chen:2020:simple} maximizes the similarity of positive pairs relative to the similarity of negative pairs. \deleted{Specifically, at each iteration, it performs randomly selected augmentations over each input to generate its ``augmented views''.} For each input $x_i$, a pair of its augmented views $(x_i, x_i^\splus)$ forms a positive pair, while a set of augmented views of other inputs $\gN_{x_i}$ form its negative pairs. 
% a mini-batch of $N$ inputs $\{x_i\}_{i=1}^N$ and performs two randomly selected augmentations on each input $x_i$ to generate a pair of augmented views $(v_i, v_i^\splus)$. 
% Let $z$ denote the latent representation of view $v$ (\mie, $z_i  = f(v_i)$).\footnote{Strictly speaking, the {\em projector}, a small multi-layer perception network, is often applied on $f(v)$ to produce $z$, which is omitted for simplicity.} The contrastive loss of the pair $(\bar{i}, \barbelow{i})$ is defined by the InfoNCE loss\cite{infonce}:
% \begin{equation}
% \hspace{-8pt}
% \label{eq:simclr}
%       \ell_{\bar{i}, \underline{i}} =  -\log\frac{\exp(\mathrm{sim}(z_{\bar{i}}, z_{\underline{i}})/\tau)}{\sum_{j \neq i}  [\,\exp(\mathrm{sim}(z_{\bar{i}}, z_{\bar{j}})/\tau) + \exp(\mathrm{sim}(z_{\bar{i}}, z_{\underline{j}}) /\tau)]} 
% \end{equation}
% where $\mathrm{sim}(\cdot, \cdot)$ is the similarity function (e.g., cosine similarity) and $\tau$ denotes the temperature parameter. The overall loss is computed over all positive pairs, both $(\bar{i}, \barbelow{i})$ and $(\barbelow{i}, \bar{i})$, in the mini-batch.
Let $z_i$ denote the latent representation of view $x_i$ (\mie, $z_i  = f(x_i)$).\footnote{Strictly speaking, the {\em projector}, a small multi-layer perception network, is often applied on $f(x_i)$ to produce $z_i$, which is omitted for simplicity.} The contrastive loss of the pair $(x_{i}, x_{i}^\splus)$ is defined by the InfoNCE loss\mcite{infonce}:
\begin{equation}
\label{eq:simclr}
%\hspace{-20pt}
      \ell_{x_i, x_i^\splus} =  -\log\frac{\exp (\frac{\mathrm{sim}(z_i, z_i^\splus )}{\tau})}
      {
      \sum_{x_j^\sminus \in \gN_{x_i}}  \exp(\frac{\mathrm{sim}(z_i, z_j^\sminus)}{\tau}) + \exp(\frac{\mathrm{sim}(z_i, z_i^\splus)}{\tau})
      } 
\end{equation}
where $\mathrm{sim}(\cdot, \cdot)$ is the similarity function (\meg, cosine similarity) and $\tau$ denotes the temperature parameter. 
%The overall loss is computed over all positive pairs, both $(x_i, )$ and $(\barbelow{i}, \bar{i})$, in the mini-batch.
% By minimizing the final loss, the encoder can align the representations of the same
% sample under different data augmentations (i.e., positive pairs),
% and  the representations of different samples (i.e.,
% negative pairs)


\vspace{1pt}
\underline{\em BYOL}\mcite{grill:2020:bootstrap} employs two asymmetric networks, the online and target networks, where the target network provides the regression target to train the online network, as illustrated in Figure\mref{figure:contra}. \deleted{Specifically, the online network (parameterized by $\theta$) consists of an encoder $f_\theta$ and a predictor $q_\theta$, while the target network (parameterized by $\vartheta$) comprises only the encoder $f_\vartheta$.} Similar to SimCLR, BYOL generates a pair of augmented views $(x_i, x_i^\splus)$ for each input and defines the contrastive loss as:
\begin{equation}
\label{eq:byol}
 \ell_{x_i, x_i^\splus} =  \| q_\theta (f_\theta(x_i))  - f_\vartheta (x_i^\splus)  \|_2^2
\end{equation}
where both $q_\theta (f_\theta(x_i))$ and $f_\vartheta (x_i^\splus)$ are $L_2$ normalized and the overall loss is symmetrized by computing over both $(x_i, x_i^\splus)$ and $(x_i^\splus, x_i)$,. The online network is optimized with respect to \meq{eq:byol}, where the stop gradient operator is applied on $f_\vartheta$; meanwhile, the target network is updated using an exponential moving average operator: 
$\vartheta = \eta \vartheta + (1 - \eta) \theta$, where $\eta$ is the moving average hyper-parameter.



% Then, BYOL  uses the mean squared error between the online network predictions and target network predictions to optimize the online network. Note that, the target network encoder is updated only through exponential moving average (EMA) from the parameters of the encoder of the online network. Specifically, the loss function can be formulated as:
% \begin{equation*}
% \begin{aligned}
%       \gL = ||q(z_i) - sg(z'_i)||^2_2 \\
%       z_i = f_\theta(v_i), \quad z'_i = f_\xi(v'_i), \\
% \end{aligned}
% \end{equation*}
% where $q$ denotes the predictor, $\xi$ is the parameter of the target network, and $sg$ denotes stop gradient operator.  The loss is only backpropagated to optimize the online network. Then, BYOL utilizes EMA to update the target network according to the following formula:
% $$\xi = \eta \xi + (1- \eta) \xi,$$
% where $\xi$ is the moving average hyperparameter.

\vspace{1pt}
\underline{\em SimSiam}\mcite{chen:2021:exploring} is a variant of BYOL, which differs mainly in removing the exponential moving average operator, as illustrated in Figure\mref{figure:contra}.

% The authors conducted an extensive evaluation and found that it is the stop gradient and the predictor that can prevent the model collapse.



\subsection{Trojan Attacks}

% With their increasing use in security-sensitive domains, DNNs become the new targets of malicious attacks, among which 

Trojan attacks represent one major threat to the security of {\dnns}\mcite{badnet, trojannn, imc, invisible-backdoor}. As illustrated in Figure\mref{fig:trojan}, the adversary plants ``backdoors'' into the victim's model during training and activates such backdoors with ``triggers'' at inference.
Typically, the infected model (trojan model) reacts to trigger-embedded inputs (trigger inputs) in a highly predictable manner (\meg, classified to the adversary's desired class) but functions normally otherwise. Formally, under the supervised setting, the loss function of trojan attacks\deleted{ via poisoning training data} is defined as:
\begin{equation}
\label{eq:trojan_sl}
\sE_{(x, y) \in  \gD}\, \ell(h(x), y)  + \lambda \sE_{x_* \in  \gD_*}\, \ell(h(x_*), t)
\end{equation}
where $\ell$ denotes the prediction loss, $\gD$ and $\gD_*$ are the clean and poisoning training data respectively, $t$ is the target class desired by the adversary, and the parameter $\lambda$ balances the influence of $\gD$ and $\gD_*$\deleted{ (\meg, by controlling their ratio)}.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.8\columnwidth]{./figures/trojan.pdf}
	\caption{\small Illustration of trojan attacks in contrastive learning. \label{fig:trojan}}
\end{figure}

Trojan attacks are of particular interest for \ssl: as \ssl-trained models are subsequently used in various downstream tasks, trojan attacks may cause widespread damage. Yet, most supervised trojan attacks are inapplicable to self-supervised learning due to label absence. Recent work has explored new ways of injecting 
backdoors into \ssl-trained models. Below, we introduce two representative attacks.


% Backdoor attack, injecting malicious functions into the victim models during the training phase, has attracted great attention recently  Most of the existing works focus on supervised learning. Generally speaking, the adversary generally first selects some poisoning examples and attaches the pre-defined trigger to them, then assigns the wrong target labels for such poisoned examples. Finally, the victim models trained on the poisoned dataset will misbehave against examples with the trigger. Formally, the poisoning process can be formulated as follows:
% \begin{equation*}
% \begin{aligned}
%      \theta^* = \min_{\theta} \mathbb{E}_{(x_i, y_i) \in  D} [\ell(x_i, y_i; \theta) ] + \mathbb{E}_{(x_i, y_i) \in  D_*} [\ell(\rho(x_i,r), y_t; \theta) ],
% \end{aligned}
% \end{equation*}
% where $\rho$ is the poisoning function. Afterward, researchers proposed some clean label backdoor attacks based on feature collision in the latent feature space \cite{Shafahi:2018:nips}. However, it is not trivial to directly extend existing backdoor attacks to the SSL setting since the label information is absent. Until recently, a few backdoor attacks against SSL are proposed.
%\noindent 



\vspace{1pt}
\underline{\em SSLBackdoor}\mcite{saha:2021:backdoor} defines a specific image patch as the trigger and generates poisoning data by attaching the patch to inputs from the target class. With random cropping, the trigger is retained in certain augmented views and removed in the others. Therefore, by aligning the positive pairs of trigger inputs, the representation of the trigger pattern is associated with the target-class inputs. \deleted{However, due to its reliance on \mct{i} whether random cropping is selected as the augmentation and \mct{ii} whether the trigger is preserved, the attack suffers a low attack success rate (\meg, $\leq 2\%$ on ImageNet-100).}


% the strong data augmentation operator (e.g., RandomCrop) may result in two augmented views for a poisoned example, one of them contains the trigger while the other not  . The adversary can associate the trigger and target class feature by poisoning the target class (i.e., attaching the trigger to the examples from the target class).

\deleted{\vspace{1pt}
\underline{\em BadEncoder}\mcite{jia:2021:badencoder} defines an objective function that associates trigger patterns with reference inputs from the target class in the representation space so that any trigger inputs are misclassified into the target class in the downstream tasks. However, compared with other self-supervised trojan attacks, BadEncoder assumes a stronger threat model in which the adversary has control over the training process. }


\vspace{1pt}
\underline{\em PoisonedEncoder}\mcite{liu:2022:poisonedencoder} targets a specific set of inputs and creates poisoning data by combining such inputs with their reference inputs in the representation space. Compared with other self-supervised trojan attacks, PoisonedEncoder is limited in that it only works on a set of pre-defined inputs rather than any trigger-embedded inputs. 

\deleted{\vspace{1pt}
Overall, the existing self-supervised trojan attacks seem to under-perform their supervised counterparts, raising the intriguing question: is \ssl inherently more resilient than supervised learning to trojan attacks? }


==> discussion.tex <==

\section{Discussion}
\label{sec:diss}




\subsection{Compared with Other Spectral Backdoor}

% We freeze a pre-trained model and only optimize a trigger end-to-end by aligning the positive pairs.  Intuitively, a pre-trained model can extract informative features of inputs. Therefore, such optimization makes the trigger pattern more invariant to random data augmentations, and further can align the trigger examples better. Besides, for stealthiness, we also add a loss term to minimize the difference between the trigger-embedded inputs and their clean counterparts. However, we observe that such trigger cannot attack successfully.  During the training, we use KNN to monitor the ASR and find that it always be close to 0. 
% Then, we consider alternatively optimizing the trigger and the model by minimizing the contrastive loss. Specifically, given a set of frequency bands, we alternatively optimize the perturbation magnitude and the model by minimizing the contrastive loss. Also, we use a loss term to limit the trigger perturbation. However, such optimization does not make the attack more effective. During the training, we use KNN to monitor the ASR and observe that it rises in the initial phase and then declines to 0 in the latter phase. We speculate that this is because the optimized trigger crafts a shortcut to decrease the contrastive loss. Therefore, the pre-trained encoder will focus more on the trigger features rather than the target class feature. How to optimize the trigger in contrastive learning is still an open question, which deserves in-depth research.








